Improving Spectrum-Based Localization of Multiple Faults by Iterative Test Suite Reduction

Spectrum-based fault localization (SBFL) works well for single-fault programs but its accuracy decays for increasing fault numbers. We present FLITSR (Fault Localization by Iterative Test Suite Reduction), a novel SBFL extension that improves the localization of a given base metric specifically in the presence of multiple faults. FLITSR iteratively selects reduced versions of the test suite that better localize the individual faults in the system. This allows it to identify and re-rank faults ranked too low by the base metric because they were masked by other program elements. We evaluated FLITSR over method-level spectra from an existing large synthetic dataset comprising 75000 variants of 15 open-source projects with up to 32 injected faults, as well as method-level and statement-level spectra from a new dataset with 326 true multi-fault versions from the Defects4J benchmark set containing up to 14 real faults. For all three spectrum types we consistently see substantial reductions of the average wasted efforts at different fault levels, of 30%-90% over the best base metric, and generally similarly large increases in precision and recall, albeit with larger variance across the underlying projects. For the method-level real faults, FLITSR also substantially outperforms GRACE, a state-of-the-art learning-based fault localizer.

==> implementation.tex <==
\section{Implementation}


==> prelim.tex <==
%\subsection{Preliminaries}
We start by defining some important concepts that will be used for the duration
of the paper.

Let $T$ denote the entire test suite, and $F$ and $P$ denote only the passing
and failing subsets of the test suite respectively. To represent the failing
tests that execute a particular program element, we give the following
definition.
\begin{definition}%
  \label{def:failset}
  We define the failing set $F(e_i)$ of a particular element $e_i$ as the set of
  all failing test cases in the test suite that execute $e_i$.
  Likewise, the passing set $P(e_i)$ denotes all passing test cases executing
  $e_i$.
\end{definition}
With this, we can now define an important concept to the FLITSR algorithm called
a \emph{span}.
\begin{definition}[Span]%
  \label{def:span}
  A \textbf{span} is a set of program elements $L$ that
  \emph{covers} all failing test cases.\ i.e. $\forall\ t_i \in F,\ \exists\ li
  \in L$ s.t. $t_i \in F(l_i)$.
\end{definition}
\begin{definition}[Basis]%
  \label{def:basis}
  Let $B$ be a \emph{span} as described in Definition~\ref{def:span}. We call
  $B$ a \textbf{basis} if $B \setminus b_i$ is not a span $\forall\ b_i \in B$.
  i.e. A basis is a minimal span, where no element can be removed and $B$ still
  a span.
\end{definition}
%TODO: fault localization invariants?

